Electrically tunable quantum confinement of neutral excitons

Confining particles to distances below their de Broglie wavelength discretizes their motional state. This fundamental effect is observed in many physical systems, ranging from electrons confined in atoms or quantum dots to ultracold atoms trapped in optical tweezers. In solid-state photonics, a long-standing goal has been to achieve fully tunable quantum confinement of optically active electron-hole pairs known as excitons. To confine excitons, existing approaches mainly rely on material modulation, which suffers from poor control over the energy and position of trapping potentials. This has severely impeded the engineering of large-scale quantum photonic systems. In this doctoral thesis, we demonstrate electrically controlled quantum confinement of neutral excitons in two-dimensional semiconductors. By combining gate-defined in-plane electric fields with inherent interactions between excitons and free charges in a lateral p-i-n junction, we achieve tunable exciton confinement lengths reaching values below 10 nm. Quantization of excitonic motion manifests in the measured optical response as a ladder of discrete voltage-dependent states below the continuum. Moreover, we observe that our confining potentials lead to a strong modification of the relative wave function of excitons. We further highlight the versatility of our approach by extending our confinement scheme to create quantum-dot-like zero-dimensional structures with a fully tunable confinement length. Our technique provides an experimental route towards achieving polariton blockade and creating scalable arrays of identical single-photon sources, which has wide-ranging implications for realizing strongly correlated photonic phases and on-chip optical quantum information processors.

==> Sources/7_Discussion.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter{Discussion and Outlook}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Limitations of field-induced confinement}
\label{discussion:limits}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The principal characteristic of our proposed technique for electrically quantum confining neutral excitons -- which we refer to as ``field-induced confinement'' --  lies in its capability to dynamically manipulate the excitonic center-of-mass (COM) confinement length. Our experimental findings suggest that an increased voltage asymmetry between gate electrodes can yield stronger gradients in the in-plane electric field, which in turn facilitate a tighter exciton confinement via the dc Stark effect. However, as we have demonstrated in chapters \ref{chap:COM} and \ref{chap:relative}, this \emph{localization in COM occurs at the expense of exciton delocalization in relative coordinates}, since the action of the electrostatic potential on electrons and holes individually is to accelerate them towards the n-doped and p-doped regions, respectively (Fig.\,\ref{fig:3_2_Confinement_scheme} \bfB). This interplay is perhaps best exemplified by the differential reflectance measurement shown in Fig.\,\ref{fig:3_10_PL_WL} \bfC. A continuous reduction in the excitonic linewidth of the lowest confined state is observed as the top gate (TG) voltage $\vtg$ is lowered, up until a point beyond which the line begins to broaden and lose oscillator strength. Evidently, as the electric field magnitude in the device increases, the exciton dissociation rate becomes a non-negligible decay channel in comparison to radiative decay. Therefore, the limiting factor impeding tighter exciton confinement clearly does not lie with the device's inability to generate larger electric fields.

To overcome this inherent limitation, a natural strategy might involve utilizing semiconductors capable of hosting excitons with even greater binding energies $E_\mathrm{B}$. Yet, the viability of this approach remains uncertain: Although the dissociation field $F_\mathrm{d}$ of such excitons would increase, their polarizability $\alpha$ would concurrently decrease, which could potentially limit the achievable dc Stark shift and, in turn, the confinement length. Alternatively, one may choose to operate with excitons in III-V semiconductors, such as in GaAs, where the binding energy is notably smaller, but the polarizability is significantly enhanced. Similarly, one might consider exploring confinement effects for Rydberg excitons in TMD semiconductors. However, considering the trade-off between polarizability $\alpha$ and dissociation field $F_\mathrm{d}$, it remains unclear as to which approach would yield the tightest exciton confinement.

This question can be addressed by considering how the polarizability $\alpha$ and dissociation field $F_\mathrm{d}$ scale with excitonic properties, such as binding energy $E_\mathrm{B}$ and Bohr radius $a_\mathrm{B}$. In Eqn.\,\ref{eqn:dissociation_field}, we have already established that the dissociation field $F_\mathrm{d} \propto \frac{E_\mathrm{B}}{a_\mathrm{B}}$. Furthermore, according to Eqn.\,\ref{eqn:polarizability}, the polarizability scales as $\alpha \propto \epsilon_r a_\mathrm{B}^3$. With these relations, it is straightforward to show that the depth $\Delta E$ of the Stark-shift-induced confinement potential scales as
\begin{equation}
    \Delta E \sim \alpha\cdot F_\mathrm{d}^2 \sim \epsilon_r a_\mathrm{B}^3 \cdot \frac{E_\mathrm{B}^2}{a_\mathrm{B}^2} \sim E_\mathrm{B}
    \label{eqn:stark_scaling}
\end{equation}
where in the last step we used Eqns.\,\ref{eqn:EB_2D} and \ref{eqn:a_B_2D}. Hence, the gain in dissociation field obtained by an increase in binding energy $E_\mathrm{B}$ outweighs the simultaneous reduction in polarizability, leading to an overall enhancement in both dc Stark shift and confinement length. Intriguingly, even though Rydberg excitons may exhibit a linear Stark shift, the same scaling behavior is recovered as in Eqn.\,\ref{eqn:stark_scaling}. Thus, while $1s$ excitons in TMD semiconductors undoubtedly represent a viable platform for developing quantum emitters using spatially modulated in-plane electric fields, our field-induced confinement technique should also be effective in other material systems, which host excitons with large binding energies, such as carbon nanotubes \cite{Ma2005,Maultzsch2005} or layered organic-inorganic perovskite crystals \cite{Yaffe2015,Saparov2016}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Minimum achievable confinement length}
\label{discussion:min_confinement_length}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Focusing on excitons in TMD van der Waals heterostructures, and in particular our proposed scheme to realize 0D excitons using split-gate electrodes (section \ref{chap:0d:sec:split-gate}), an immediate question follows: What is the minimum achievable confinement length in this setting? To address this question, we consider a simplified version of this device geometry, shown in Fig.\,\ref{fig:pn_model_geometry}, which consists only of a pair of split bottom gate (BG) electrodes, a dielectric spacer and a monolayer semiconductor, in which charges are injected through electrostatic doping. To increase the in-plane field magnitude in the TMD and thus achieve a tighter exciton confinement, a natural approach would be to reduce both, the thickness $t$ of the h-BN spacer layer and the gap size $l_\mathrm{gap}$ between the split-gate electrodes. The h-BN thickness could be reduced up to $4\,$nm, beyond which the dielectric breakdown field would limit the achievable charge densities in the TMD. Furthermore, by improving the electron beam lithography (EBL) process, the gap size $l_\mathrm{gap}$ could be reduced to approximately $20\,$nm. In spite of these modifications, the best achievable confinement length $\ell_x$ would remain at around $6\,$nm. The main issue thereby lies in the inability of our confinement scheme to allow for independent tuning of the confinement potential depth and its stiffness. In the example above, exciton dissociation places an upper bound on the tolerable dc Stark shift, which in turn limits the minimum achievable confinement length.

\begin{figure}[htb]
    \centering
	\includegraphics[width=10.5cm]{Figures/Ch7_pn_model_geometry.pdf}
	\caption{\textbf{2D gate-tunable lateral p-n junction.}
    The modelled device geometry consists of a pair of split bottom gate electrodes BG-L and BG-R, with applied biases $V_\mathrm{L}$ and $V_\mathrm{R}$ respectively. The monolayer semiconductor is placed atop a h-BN spacer layer with thickness $t$. By choosing $V_\mathrm{L} = -V_\mathrm{R}$ a p-n junction in the TMD is formed with a depletion region of width $d$.
    }  
	\label{fig:pn_model_geometry}
\end{figure}

To understand how the potential depth and stiffness can be decoupled from each other, we need to delve deeper into the electrostatics of a 2D gate-tunable lateral p-n junction \cite{Chaves2023}. This will allow us to determine how these parameters are linked to the material and geometric attributes of the device. To make the problem analytically more tractable we solve the 2D Poisson equation and determine the electrostatic potential solely within the depletion region of the device shown in Fig.\,\ref{fig:pn_model_geometry}. This simplification is motivated by the assumption that in-plane variations of the electrostatic potential will be negligible outside of this region compared to within. For the moment, we consider the dimensions of the device along the $y$-axis to be long enough, such that the system can be considered translationally invariant in that direction. At the bottom of the device structure, the potential $\phi = \phi_g(x)$ is defined by the split BG electrodes, which constitutes a Dirichlet boundary condition (BC). For simplicity, we assume the physical gap between the two electrodes to be infinitesimally small, such that the potential across the gates changes abruptly:
\begin{equation}
    \phi_g(x) = 
        \begin{cases}
            V_\mathrm{L},  & 0 \leq x < d/2, \\
            V_\mathrm{R},  & d/2 \leq x \leq d
        \end{cases}
\end{equation}
where $V_\mathrm{L/R}$ is the potential applied to the left and right BG, respectively. This should enable us to establish a conservative estimate for the minimum possible width of the depletion zone. On the left ($x=0$) and right ($x=d$) side of the structure, homogeneous Neumann BCs are imposed, which drive the in-plane electric field to zero outside the depletion area i.e.\,$\frac{\partial \phi}{\partial x}=0$. To account for the surface charge associated with the monolayer semiconductor, a non-homogeneous Neumann BC is set at the top surface i.e.\,$\frac{\partial \phi}{\partial z}=\sigma(x)/\epsilon$. $\sigma(x)$ is the surface charge density given by $q(p(x)-n(x))$, where $p(x)$ and $n(x)$ are hole and electron densities, respectively. $\epsilon$ represents the dielectric permittivity of the insulating spacer layer. However, since only the depletion region is considered, the net charge density in the semiconductor is zero and the problem reduces from solving a 2D Poisson equation to a 2D Laplace equation ($\nabla^2\phi=0$).
We perform a separation-of-variables ansatz, $\phi(x,z)=X(x)\cdot Z(z)$, such that the Laplace equation reads
\begin{equation}
    Z\frac{d^2 X}{dx^2} + X\frac{d^2 Z}{dz^2} = 0
\end{equation}
Dividing by $\phi$ gives rise to two separate ordinary differential equations
\begin{subequations}
    \begin{align} 
        \frac{d^2 X}{dx^2} + \lambda^2 X &=  0, \\ 
        \frac{d^2 Z}{dz^2} - \lambda^2 Z &=  0,
    \end{align}
\end{subequations}
where we consider the case $\lambda^2>0$ without loss of generality. The solutions of these equations expressed in their most general form are
\begin{subequations}
    \begin{align} 
        X(x) &=  a_k\sin(\lambda_k x) + b_k \cos(\lambda_k x), \\ 
        Z(z) &=  c_k\exp(-\lambda_k z) + d_k\exp(\lambda_k z)
    \end{align}
\end{subequations}
The Neumann BCs at the left $\left(\frac{\partial \phi}{\partial x}\bigr|_{x=0}=0\right)$ and right edge $\left(\frac{\partial \phi}{\partial x}\bigr|_{x=d}=0\right)$ lead to $a_k=0$ and $\sin(\lambda_k d)=0$, respectively. The latter sets $\lambda_k=\frac{k\pi}{d}$ with $k=1,2,3,\ldots,$ such that
\begin{equation}
    X(x) = b_k\cos\left(\frac{k\pi}{d} x\right)
\end{equation}
Similarly, the Neumann BC at the top surface $\left(\frac{\partial \phi}{\partial z}\bigr|_{z=t}=0\right)$ gives rise to $c_k = d_k\exp(2\lambda_k t)$, which in turn yields
\begin{equation}
    Z(z) = 2d_k\exp(\lambda_k t)\cosh\left(\lambda_k(t-z)\right)
\end{equation}
Hence, the electrostatic potential in its most general form can be denoted as
\begin{equation}
    \phi(x,z)=\sum_{k=1}^{\infty} A_k \cos\left(\lambda_k x\right) \cosh\left(\lambda_k(t-z)\right)
\end{equation}
To determine the value of $A_k$ the Dirichlet BC at the bottom interface $\left(\phi(x,z=0) = \phi_g(x)\right)$ can be used
\begin{equation}
    \phi_g(x) = \sum_{k=1}^{\infty} A_k \cosh\left(\lambda_k t\right) \cos\left(\lambda_k x\right)
\end{equation}
which represents a Fourier series for the potential applied at the split BG electrode $\phi_g(x)$. Correspondingly,
\begin{equation}
    A_k = \frac{\int_{0}^{d}\phi_g(x)\cos\left(\lambda_k x\right)\, dx}{\cosh\left(\lambda_k t\right) \int_{0}^{d}\cos^2\left(\lambda_k x\right)\, dx}
\end{equation}
Under symmetric biasing conditions, i.e.\,$V_\mathrm{L} = -V_\mathrm{R}$, the integral in the numerator can be evaluated as
\begin{equation}
\begin{split}
    \int_{0}^{d}\phi_g(x)\cos\left(\lambda_k x\right)\, dx &= \int_{0}^{d/2} V_\mathrm{L}\cos\left(\lambda_k x\right)\, dx - \int_{d/2}^{d} V_\mathrm{L}\cos\left(\lambda_k x\right)\, dx \\
    &= \frac{2 V_\mathrm{L}}{\lambda_k} \sin\left(\lambda_k \frac{d}{2} \right)
\end{split}
\end{equation}
Hence, the coefficients $A_k$ are given by
\begin{equation}
    A_k = \frac{4 V_\mathrm{L}}{\lambda_k d} \frac{\sin\left(\lambda_k \frac{d}{2} \right)}{\cosh (\lambda_k t)}
\end{equation}
To obtain an expression for the width of the depletion region, we can evaluate the electrostatic potential at the top interface. The monolayer semiconductor is p-doped to the left, and n-doped to the right of the depletion region. Hence, the potential at the left edge of the semiconductor will approximately coincide with the semiconductor valence band edge i.e.\,$\phi(0,t) \approx -E_\mathrm{g}/2$, where $E_\mathrm{g}$ is the semiconductor bandgap. Therefore,
\begin{equation}
\begin{split}
    \phi(0,t) &= \sum_{k=1}^{\infty} A_k = \sum_{k=1}^{\infty} \frac{4 V_\mathrm{L}}{k \pi} \frac{\sin\left(\frac{k\pi}{2} \right)}{\cosh\left(k\pi\frac{t}{d} \right)} \\
    &\approx -E_\mathrm{g}/2,
\end{split}
\end{equation}
which constitutes a nonlinear equation for determining $d$. As a simplification, we consider only the first term in the sum ($k=1$), from which $d$ can be approximated as
\begin{equation}
    d \approx \frac{\pi}{\mathrm{cosh}^{-1}\left( \frac{8}{\pi} \frac{|V_\mathrm{L}|}{E_\mathrm{g}} \right)} \cdot t
\end{equation}
Similarly, the maximum of the in-plane electric field $F_\mathrm{x,max}$ can be approximated by taking the derivative of the electrostatic potential, inserting the above expression and considering only the first term of the sum:
\begin{equation}
    F_\mathrm{x,max} = \frac{\partial \phi}{\partial x}\bigg|_{x=d/2} \approx \frac{\pi}{2} \frac{E_\mathrm{g}}{d}
    \label{eqn:fx_max}
\end{equation}
To verify the predictive accuracy of these expressions, we simulate the device geometry in Fig.\,\ref{fig:pn_model_geometry} using a numerical solver (using procedures described in detail in section \ref{sec:1DX_sims}) for three different thicknesses of the h-BN spacer layer ($30\,$nm, $20\,$nm and $10\,$nm), assuming symmetric biasing conditions $V_\mathrm{L}=-V_\mathrm{R}$ throughout. A comparison of the calculated and simulated values is shown in Fig.\,\ref{fig:pn_model_predictions} as a function of the hole charge density in the p-doped region. As the charge densities increase, the predicted values of the depletion width $d$ tend to agree better with the results derived from simulations. This behavior can be attributed to our BCs which impose a zero in-plane electric field at the left and right edges of the depletion zone, an assumption that increasingly holds as the charge densities in the TMD monolayer increase.
On the other hand, the predicted values of the electric field maxima $F_\mathrm{x,max}$ evolve in a manner very similar to those extracted from the simulations, albeit while overestimating them approximately by $30\%$. As such, a good fit with the approximate expression in Eqn.\,\ref{eqn:fx_max} can be obtained by including an empirical correction factor in the term.

\begin{figure}[htb]
    \centering
	\includegraphics[width=12cm]{Figures/Ch7_pn_model.pdf}
	\caption{\textbf{Validity of approximate model of a 2D p-n junction.}
    To verify the validity of the approximate expressions derived for the depletion width $d$ and in-plane electric field maximum $F_\mathrm{x,max}$, we simulate the device geometry in Fig.\,\ref{fig:pn_model_geometry} using a numerical solver for three different thicknesses of the h-BN spacer layer: $30\,$nm (circles), $20\,$nm (triangles) and $10\,$nm (squares), for a series of gate voltages $V_\mathrm{L}$ and assume symmetric biasing conditions $V_\mathrm{L}=-V_\mathrm{R}$. (\bfA) Comparison of the calculated (blue) with the simulated results (black) are shown in (\bfA) for the depletion width $d$ and (\bfB) for the in-plane electric field maximum $F_\mathrm{x,max}$. These quantities are plotted as a function of the hole charge density in the p-doped region.
    }  
	\label{fig:pn_model_predictions}
\end{figure}

Having determined analytical expressions for the depletion width and the in-plane electric field distribution in the TMD monolayer, and having verified their validity through numerical simulations, it is possible to now derive an approximate expression for the exciton confinement length $\ell_x$
\begin{equation}
    \ell_x = \sqrt{\frac{\hbar}{m\omega}} = \frac{d}{\pi}\sqrt{\frac{2\hbar}{E_\mathrm{g}}} \frac{1}{(m\alpha)^{1/4}}
    \label{eqn:lx_approximation}
\end{equation}
To keep the depth of the confinement potential fixed while reducing the confinement length, we need to compare Eqns.\,\ref{eqn:fx_max} and \ref{eqn:lx_approximation}. Evidently, a sole reduction of the dielectric thickness $t$ will not be beneficial, since $F_\mathrm{x,max} \propto 1/t$ while $\ell_x \propto t$. However, a closer inspection of the two expressions reveals a varying dependence on the bandgap $E_\mathrm{g}$: While the electric field maximum directly scales with the bandgap, $F_\mathrm{x,max} \propto E_\mathrm{g}$, the confinement length scales inversely with the square root of the bandgap $\ell_x \propto 1/\sqrt{E_\mathrm{g}}$. Therefore, if a reduction in h-BN thickness $t$ is accompanied by a reduction in the bandgap $E_\mathrm{g}$, $F_\mathrm{x,max}$ can be kept at a constant value, while simultaneously allowing for a tighter exciton confinement.

In principle, this suggests the incorporation of a smaller bandgap semiconductor in our device architecture, which is undesirable since such materials typically also host excitons with reduced binding energies. Hence, as an alternative, we propose to consider a TMD hetero-bilayer system consisting of a MoSe$_2$ monolayer and another TMD $M\!X_2$ in a type-II band alignment configuration, which gives rise to an effective bandgap $E_\mathrm{g,eff}$ smaller than the MoSe$_2$ bandgap (Fig.\,\ref{fig:pn_reduced_EG} \bfA). To prevent layer hybridization or interlayer exciton formation, a h-BN spacer layer between the two semiconductors is included. In such a configuration, when BG-L and BG-R are oppositely biased ($V_\mathrm{L} = -V_\mathrm{R}$) to form a p-n junction, holes are injected only in the MoSe$_2$ layer and electron injection occurs solely in the $M\!X_2$ layer. To put this proposal to the test, we simulate a device structure as shown in Fig.\,\ref{fig:pn_reduced_EG} \bfB, while assuming a thickness of $4\,$nm for both h-BN layers and a gap size $l_\mathrm{gap}$ of $20\,$nm between the split-gate electrodes. For the second TMD layer we use the material HfS$_2$, since its conduction band edge is well aligned with the valence band edge of MoSe$_2$, giving rise to an effective bandgap $E_\mathrm{g,eff}$ of approximately $0.6\,$eV according to DFT simulations \cite{Haastrup2018}. The resulting excitonic confinement potential is illustrated in Fig.\,\ref{fig:pn_reduced_EG} \bfC. A device consisting of a bare MoSe$_2$ monolayer (black curve) will exhibit an excitonic confinement length of approximately $6\,$nm, as established earlier. However, by switching to the hetero-bilayer system (blue curve), the potential depth can be maintained while reducing the confinement length to approximately $4\,$nm.

In all our considerations above, the focus thus far has primarily been on the confinement length $\ell_x$ along the $x$ direction. As demonstrated in Fig.\,\ref{fig:confinement_split-gate}, the confinement length $\ell_y$ along the $y$ direction is directly proportional to the width $d_y$ of the split-gate electrodes. Therefore, minimizing $\ell_y$ necessitates a reduction in width $d_y$. Standard EBL processes will not enable lowering $d_y$ beyond $20\,$nm. To overcome this limitation, we propose an intriguing alternative to patterned metallic electrodes: using a carbon nanotube as a gate, which can be etched to define two separate halves, thus forming a split-gate. Based on our numerical simulations, this approach could potentially yield a confinement length $\ell_y$ close to $3\,$nm. Therefore, by integrating these strategies, our analysis points to a minimum achievable excitonic confinement area of $\ell_x \cdot \ell_y\sim 10\,$nm$^2$.

\begin{figure}[htb]
    \centering
	\includegraphics[width=14cm]{Figures/Ch7_pn_reduced_EG.pdf}
	\caption{\textbf{Decrease in confinement length through reduction in effective band gap.}
    (\bfA) We consider a TMD hetero-bilayer system consisting of a MoSe$_2$ monolayer and another TMD $M\!X_2$ in a type-II band alignment configuration, which gives rise to an effective bandgap $E_\mathrm{g,eff}$ smaller than the MoSe$_2$ bandgap (\bfB) Upon formation of a p-n junction, holes are injected in the MoSe$_2$ and electrons in the $M\!X_2$ layer. (\bfC) A device consisting of a single MoSe$_2$ monolayer (black curve) will exhibit an excitonic confinement length of approximately $6\,$nm. By switching to the hetero-bilayer system (blue curve), the potential depth can be maintained while reducing the confinement length to approximately $4\,$nm.
    }  
	\label{fig:pn_reduced_EG}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Towards polariton blockade}
\label{discussion:blockade}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Trapping excitons on such tight confinement length scales allows us to drastically boost the anharmonicity of the quantum emitter. This gain, however, comes at the expense of a dramatically reduced scattering cross-section with photons, owing to the mismatch between excitonic and photonic mode volumes (see Eqn. \ref{eqn:exc_phot_mode_overlap}). Therefore, achieving a deterministic emitter-photon interaction becomes progressively more challenging as the confinement length is reduced, which effectively turns the emitter into an inefficient source of single photons. To improve the photon extraction efficiency in such cases and enhance the overall light--matter coupling, one possible strategy is to additionally confine the electromagnetic field to subwavelength volumes using optical cavities. As a consequence, the spontaneous emission rate $\gamma_\mathrm{sp}$ of the emitter will be amplified by the Purcell factor $F_\mathrm{p}$, which is inversely proportional to the mode volume of the optical cavity. Moreover, by enhancing the radiative decay over all other dephasing rates in the system, the indistinguishability of single-photon emission can be improved. Hence, by augmenting the light--matter interaction $g$, significant improvements can be achieved in both the brightness and coherence properties of the emitter \cite{Turunen2022}.

If the light--matter coupling $g$, corresponding to the rate of energy exchange between cavity photons and excitons, exceeds their respective decay and decoherence rates, the combined system is adequately described in terms of new elementary excitations, termed polaritons \cite{Deng2010,Carusotto2013,Kavokin2017}. Tuning the cavity energy $E_\mathrm{cav}$ into resonance with the excitonic transition $E_\mathrm{exc}$, leads to creation of an upper and lower polariton state, which are detuned from $E_\mathrm{cav} = E_\mathrm{exc}$ by $+g$ and $-g$, respectively, an effect known as strong coupling. In the following, we exclusively focus on the lower polariton state $\hat{p}$ which, being a hybrid light--matter excitation, can be described as a superposition of photonic and excitonic constituents
\begin{equation}
    \hat{p} = c_\mathrm{p} \hat{a} + c_\mathrm{x} \hat{x}
\end{equation}
where $\hat{a}$ and $\hat{x}$ are cavity photon and exciton annihilation operators (section \ref{chap:theory:sec:LM_coupling}), respectively, with $c_\mathrm{p}$ and $c_\mathrm{x}$ being the corresponding Hopfield coefficients which satisfy $\left|c_\mathrm{p} \right|^2 + \left|c_\mathrm{x} \right|^2 = 1$. Thus, the photon (exciton) fraction of the polariton state is given by $\left|c_\mathrm{p} \right|^2$ ($\left|c_\mathrm{x} \right|^2$).

Achieving strong photon--photon interactions by varying the degree of exciton confinement \cite{Verger2006} in such a system requires careful consideration of the interplay between exciton--exciton interaction strength $U$ and the light--matter coupling strength $g$. While decreasing the confinement length from the ``quantum-well limit'', corresponding to $\ell_x \sim 100\,$nm, the polariton--polariton nonlinearity will be given by $\left|c_\mathrm{x} \right|^4 \cdot U$ \cite{Carusotto2013,Delteil2019}. Conversely, while increasing the confinement length from the ``quantum-dot limit'', defined by $\ell_x \sim 1\,$nm, the Jaynes–Cummings nonlinearity will hold, given by $(2-\sqrt{2}) \cdot g$ \cite{Carusotto2013}. Additionally, we underscore that both $U$ and $g$ are not fixed quantities and can be influenced by the degree of exciton localization. The interaction strength $U$ will scale $\propto 1/A_\mathrm{exc} = 1/\ell_x^2$ (section \ref{chap:0d:sec:intro}), where $A_\mathrm{exc}$ is excitonic COM area and we assume an isotropic emitter for simplicity. Conversely, the light--matter coupling $g$ exhibits a scaling $\propto \sqrt{A_\mathrm{exc}} = \ell_x$ (section \ref{chap:theory:sec:LM_coupling}). These disparate scaling relations highlight a critical point: as the confinement length is varied, a crossover will occur between the two regimes, setting a maximum attainable photon--photon interaction strength in the hybrid light--matter system. Specifically, towards the quantum-well limit, the anharmonicity of the quantum emitter is insufficient to introduce substantial nonlinearity to photons. In contrast, near the quantum-dot limit, the emitter exhibits pronounced anharmonicity, yet the diminished light--matter coupling $g$ impedes an efficient coupling between the cavity photon and the emitter.

We have visualized this interplay in Fig.\,\ref{fig:U_vs_g}, which shows the dependence of the exciton--exciton interaction strength and the light--matter coupling on the exciton confinement length $\ell_x$. Here, we assumed $U = \overline{U}/A_\mathrm{exc}$ with the background interaction parameter $\overline{U} \sim 0.1\,\mu$eV\,$\mu$m$^2$ \cite{Barachati2018,Scuri2018,Tan2020,Uto2023} and $g \sim 15\,$meV, a value typical for 2D excitons in TMD monolayers embedded in a 0D open microcavity structure \cite{Sidler2017,Tan2020}, as the one illustrated in Fig.\,\ref{fig:0d_dot_cavity} \bfC. Reaching polariton blockade in this system requires both $U$ and $g$ to exceed the dissipation rate $\gamma$ of the hybrid light--matter system, which we have set to $100\,\mu$eV. This condition defines a finite range of confinement lengths over which blockade can be achieved, ranging from approximately $5\,$nm to $20\,$nm. Notably, a clear maximum in photon--photon interactions materializes at a confinement length close to $10\,$nm, a value well compatible with our confinement method.

Moveover, Fig.\,\ref{fig:U_vs_g} also highlights the immense challenge in achieving polariton blockade with an isolated self-assembled quantum dot. By fixing the exciton COM confinement length to a regime in which light--matter coupling is inherently poor, blockade can only be achieved by a significant reduction in dissipation rates. Experimentally, this demands a high cavity finesse while concurrently ensuring that the quantum dot is positioned accurately with respect to the cavity mode profile. Such stringent requirements represent a formidable challenge to the scalability of these systems. In contrast, if the constraint on a fixed COM confinement length were to be relaxed -- as is feasible with our technique -- the excitonic emitter can be brought into a regime of improved light--matter interaction, consequently permitting considerably relaxed experimental conditions.

\begin{figure}[htb]
    \centering
	\includegraphics[width=10cm]{Figures/Ch7_U_vs_g.pdf}
	\caption{\textbf{Conditions for reaching polariton blockade.}
    Exciton--exciton interaction shift $U$ (green) and light--matter coupling strength $g$ (blue) for an isotropic quantum confined exciton state. Conditions for polariton blockade are met when both $U$ and $g$ exceed the dissipation rate $\gamma$ (dashed black line), assumed to be $100\,\mu$eV. This is achieved over a finite range of confinement lengths, ranging from approximately $5\,$nm to $20\,$nm. For confinement lengths exceeding $20\,$nm the anharmonicity of the quantum emitter is insufficient to introduce substantial nonlinearity to photons. For values below $5\,$nm the emitter exhibits pronounced anharmonicity, however, the diminished light--matter coupling $g$ prevents an efficient cavity photon-emitter interaction.
    }  
	\label{fig:U_vs_g}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Integration with optical cavities}
\label{discussion:cavity_integration}
\renewcommand{\thefootnote}{\arabic{footnote}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Developing strategies for interfacing excitons in 2D semiconductors with optical cavities has remained a vibrant area of research for years. In this section, our aim is not to offer an exhaustive review of such techniques. Rather, we emphasize that our confinement scheme crucially relies on creating a spatially varying electrostatic potential in the TMD monolayer, achieved through gate electrodes. It is the incorporation of these metallic layers in optical cavities that deserves special attention, as neglecting this aspect could result in substantial absorption losses, thereby greatly increasing the difficulty of observing polariton blockade.

Considering a dual-gated TMD heterostructure within a 0D open microcavity architecture, a viable strategy could involve positioning graphene gate electrodes at the nodes of the cavity electric field \cite{Tan2022}, a method already proven effective in charge-tunable III-V heterostructures \cite{Najer2019}. The TMD monolayer is thereby placed in the field anti-node to maximize light--matter interaction strength $g$. A potential limitation, however, lies in the resulting constraint for h-BN spacers to maintain a thickness of $86\,$nm, which corresponds to $\lambda/4n_\mathrm{h-BN}$, with $n_\mathrm{h-BN}$ being the \mbox{h-BN} refractive index of 2.2 at a wavelength $\lambda=760\,$nm\footnote{This wavelength corresponds to the neutral exciton transition in monolayer MoSe$_2$.}. Consequently, the main concern is that increasing the h-BN thickness to these values might significantly restrict the highest attainable in-plane electric field strength, and subsequently, the confinement length in the device (see also section \ref{discussion:min_confinement_length}).

To investigate the effect of such thick h-BN on quantum-confined states we fabricated Device 7, an optical micrograph of which is shown in Fig.\,\ref{fig:device_7} \bfA. The MoSe$_2$ monolayer is encapsulated by h-BN dielectrics with a thickness of $86\,$nm, which is verified with AFM prior to device fabrication. The gate electrodes along with the contact to the MoSe$_2$ monolayer are made of few-layer graphene, which are connected to metal electrodes formed with Ti/Au ($5\,$nm/$85\,$nm). The TG and BG only feature a partial spatial overlap (Fig.\,\ref{fig:device_7} \bfB), such that 1D quantum-confined states can be created along the TG edge. The entire heterostructure is placed on a distributed Bragg reflector (DBR) substrate. Additional details about the fabrication procedure can be found in appendix section \ref{appendix:fabrication}.

\begin{figure}[htbp]
    \centering
	\includegraphics[width=14cm]{Figures/Ch7_Device_DBR.pdf}
	\caption{\textbf{Signatures of quantum confined excitons in Device 7.}
    (\bfA) Optical micrographs of Device 7. The white dashed line indicates the monolayer MoSe$_2$ flake, which is contacted by few-layer graphene (black dashed line) and encapsulated in h-BN. The TG (blue dashed line) and BG are also made of few-layer graphene. While the TG only partially covers the MoSe$_2$ monolayer, the BG extends across the entire depicted area of the figure. The entire heterostructure is placed on a DBR substrate. The scale bar denotes $10\,\mu$m. (\bfB) Schematic illustration of the device architecture. The h-BN dielectric spacers are chosen to be $86\,$nm thick, which corresponds to $\lambda/4n_\mathrm{h-BN}$, $n_\mathrm{h-BN}$ being the h-BN refractive index of 2.2 at a wavelength $\lambda=760\,$nm. In this manner, both gate electrodes lie in the node of the cavity electric field, while the MoSe$_2$ monolayer is placed in the anti-node. (\bfC) Normalized differential reflectance $\Delta R/R$ as a function of $\vtg$, measured on the TG edge at $\vbg = 2\,$V outside the microcavity. In addition to the typical features associated with the neutral exciton (X$_\mathrm{2D}$) and polaron branches (RP$^\pm$ and AP$^\pm$) from underneath the TG, three quantum-confined states $\xqc$ are visible. (\bfD) Reflectance spectrum taken at $\vtg=-16.8\,$V.
    }  
	\label{fig:device_7}
\end{figure}

In Fig.\,\ref{fig:device_7} \bfC, we depict the normalized differential reflectance $\Delta R/R$ of the heterostructure as a function of $\vtg$ and fixed $\vbg=2\,$V outside the microcavity. In addition to the typical features associated with the neutral exciton (X$_\mathrm{2D}$) and polaron branches (RP$^\pm$ and AP$^\pm$) from underneath the TG, three distinct quantum-confined states $\xqc$ are visible. Looking at the reflectance spectrum taken at $\vtg=-16.8\,$V (Fig.\,\ref{fig:device_7} \bfD), a level splitting of approximately $1.5\,$meV can be deduced, indicative of a confinement length $\ell_x$ close to $10\,$nm. Rather than confirming our previous concerns, these findings suggest highly conducive conditions for reaching the blockade regime, as demonstrated in Fig.\,\ref{fig:U_vs_g}. Hence, as part of ongoing research efforts, we aim to apply the 0D exciton creation strategies from the preceding chapter to such device architectures, in the pursuit of demonstrating polariton blockade. We note that the requisite patterning of graphene gate electrodes into a split-gate geometry can also be accomplished with an EBL process, combined with RIE etching (appendix section \ref{appendix:fabrication}). Alternatively, for a resist-free and thus cleaner approach, we propose employing local anodic oxidation techniques, which utilize a conductive AFM tip in a humid environment to locally etch features in graphene \cite{Li2018,Cohen2023}.

While the demonstration of a polariton blockade in this system would indeed be a significant achievement, extending this scheme to create arrays of quantum emitters, each individually strongly coupled to a cavity mode, poses an appreciable challenge. In this regard, we briefly comment on three potential strategies that we believe may yield promising results. To overcome the limitations of current 0D microcavity systems, we have developed an approach to create arbitrary photonic potential landscapes, which rely on freeform patterned h-BN \cite{Lassaline2021} using thermal scanning probe lithography (tSPL) \cite{Howell2020,Albisetti2022}. In this manner, by shaping h-BN layers in the form of a parabolic lens and placing it in between two flat DBR mirrors, we realized a 0D cavity mode with a Q-factor approaching $10^4$. Owing to the versatility of tSPL, this approach can readily be extended to create arrays of tunnel-coupled cavities. In addition, the use of h-BN-based structures simplifies their integration with van der Waals heterostructures greatly.

Another promising avenue involves the utilization of hybrid plasmonic-photonic resonators, credited with merging the advantages of plasmonic structures (subwavelength mode confinement) and dielectric microcavities (high quality factors) \cite{Doeleman2016,Palstra2019,Zhang2020,Doeleman2020}. One potential implementation might involve hybridizing cavity modes in a gold, plasmonic bow-tie antenna and a photonic crystal nanobeam cavity, which could be fabricated in h-BN itself \cite{Kim2018,Nonahal2023}. Such hybrid architectures are projected to achieve quality factors around $10^4$, while preserving a mode volume of approximately $10^{-1}\,(\lambda/n)^3$. The appeal of such structures lies in the potential dual function of the plasmonic bow-tie antenna, which could concurrently serve as a split-gate electrode, enabling excitonic confinement precisely at a location where the electric field of the cavity mode is at its maximum.

Finally, we believe new opportunities could be unlocked by completely discarding the use of metallic gate electrodes in our device architectures. Instead, we propose an integration of TMD heterostructures with ferroelectric materials. Their built-in polarization could be utilized to create spatially modulated electrostatic potential landscapes in TMDs, and notably p-n junctions \cite{Chen2018,Wen2019,Lv2019,Wu2020,Wu2020a,Fraunie2023}. Suitable material candidates for this purpose are lithium niobate (LN) \cite{Wen2019} or scandium-doped aluminum nidride (AlScN) \cite{Wang2023,Kim2023}, among others.
The advantages of adopting this strategy are twofold. First, the upscale of our experimental platform could benefit significantly from the extensive fabrication expertise accrued in two well-established fields in which ferroelectrics serve a key role -- integrated photonics \cite{Zhu2021} and nonvolatile memory devices \cite{Jin2022}. Second, although such device architectures would not permit an in-situ electric tunability of confinement potentials, they offer a notable benefit: the ability to generate localized domains in the ferroelectric material with sizes down to few tens of nanometers using local stimuli \cite{Li2008}, such as electric fields applied with a conductive scanning probe tip. In this manner a truly continuously varying modulation of the electrostatic potential in space $V(x,y)$ can be achieved. 

\vspace{1cm}

\PRLsep

\vspace{1cm}

In summary, we have demonstrated a method to achieve electrically controlled quantum confinement of neutral excitons in monolayer TMD semiconductors, which offers several crucial design advantages over material modulation approaches, such as band-gap engineering, moir\'{e} potentials and strain engineering. Excitonic confinement potentials can be deterministically positioned through the appropriate design of gate electrodes and dynamically tuned by modifying the applied gate voltages. Consequently, the resonance energy of confined exciton states can be electrically tuned, allowing to correct for spatial disorder and thus create identical quantum emitters. Furthermore, quantum confinement of in-plane direct excitons is achieved, as opposed to layer-indirect excitons, which can facilitate strong coupling to light. Such tunable quantum confined systems are expected to exhibit strongly enhanced exciton--exciton interactions \cite{Li2020,Kremser2020,Baek2020}, while concurrently allowing hybridization with an optical cavity or waveguide mode \cite{Rosenberg2018,Togan2018,Lodahl2015}. Our experimental platform could therefore emerge as a building block of a strongly interacting many-body photonic system \cite{Chang2014,Carusotto2013,Noh2016}, and enable the investigation of correlated phases such as a 1D Tonks-Girardeau gas \cite{Carusotto2009,Oldziejewski2022} or a bosonic Mott-insulator of exciton-polaritons \cite{Hartmann2006,Greentree2006}.


